Canonical Surface Mapping via Geometric Cycle Consistency

We explore the task of Canonical Surface Mapping (CSM). Specifically, given an image, we learn to map pixels on the object to their corresponding locations on an abstract 3D model of the category. But how do we learn such a mapping? A supervised approach would require extensive manual labeling which is not scalable beyond a few hand-picked categories. Our key insight is that the CSM task (pixel to 3D), when combined with 3D projection (3D to pixel), completes a cycle. Hence, we can exploit a geometric cycle consistency loss, thereby allowing us to forgo the dense manual supervision. Our approach allows us to train a CSM model for a diverse set of classes, without sparse or dense keypoint annotation, by leveraging only foreground mask labels for training. We show that our predictions also allow us to infer dense correspondence between two images, and compare the performance of our approach against several methods that predict correspondence by leveraging varying amount of supervision.

==> results/pck_apk_old.tex <==
\begin{table}[h]
\setlength{\tabcolsep}{5pt} 
\centering 
% \small{
% \scalebox{1.0}{
\resizebox{\ifdim\width>\columnwidth
        \columnwidth
      \else
        \width
      \fi}{!}{
  \begin{tabular}{l l  l  l l l}
    % \toprule
    \toprule
    \toprule
    Annotation & Method & \multicolumn{2}{c}{Birds} & \multicolumn{2}{c}{Cars}\\

     &  & PCK & APK & PCK & APK\\
    \midrule
    % \hline
    KP + Seg. Mask & CMR \cite{cmrKanazawa18} & 46.9 & 20.3 & 45.4 & 18.0    \\
    % \hline
    \midrule
    Pose  + Syn. Data & Zhou et. al \cite{zhou2016learning} & - & - & 37.1 & 10.5  \\ 
    % & & & \\
    % Naive Baseline w pose & 50.1 & 48.9 \\
    Pose + Seg. Mask & CSM (ours) w/ pose & 56.6 & 31.6 & 53.0 & 22.4 \\
    \midrule
     \multirow{3}{*}{Seg. Mask}&  Dense Equi \cite{thewlis2017unsupervised}  & 34.8 & 11.2 & 31.6 & 5.7   \\
    % Naive Baseline w\/o pose & 20.9 & 31.3 \\
    & VGG Transfer \cite{long2014convnets} & 17.2 & 2.6   & 11.7 & 0.7  \\
    & CSM (ours)            & 47.7 & 23.1  & 35.5 & 8.5  \\
    \bottomrule \bottomrule
\end{tabular}
}
% }
\vspace{-0.1in}
\caption{{\bf PCK and APK}. Percentage of correct keypoints (PCK) and Keypoint Transfer AP (APK) at $\alpha=0.1$.  See Section \ref{subsec:eval-metrics} for metric descriptions. All evaluations are on 10000 image pairs per category. Higher is better. 
% The best numbers are in \textbf{bold}.
}
\label{tab:pck}
\end{table}

==> results/visibility.tex <==
\begin{table}[h]
\setlength{\tabcolsep}{0.3em} 
\centering 
\footnotesize{
\scalebox{1.0}{
  \begin{tabular}{c|ccc}
    \toprule
    Method & Birds& Cars & Airplanes\\
    \midrule
    CMR & 38.9 & 59.4  & -   \\
    \midrule
    Zhou et. al & -  & - & - \\
    Naive Baseline w pose & 42.6 & 60.8 & - \\
    Ours w/ pose & 48.3 & 60.9 & - \\
    \midrule
    Ours w/o pose            & 40.8 & 55.4 & - \\
    Naive Baseline w\/o pose & 19.6 & 46.5 &- \\
    Dense Equi  & 28.5 & 55.0 & - \\
    VGG pretrain & 19.6  & 55.45 & - 
\end{tabular}
}
}
\vspace{-0.1in}
\caption{Visibility evaluations Mean PCK at $\alpha=0.1$, across all keypoints. Evaluated on 10000 pairs of objects.
% The best numbers are in \textbf{bold}.
}
\label{tab:gt-boxes}
\end{table}

==> visuals/birds2.tex <==
\begin{table*}[!h]
\setlength{\tabcolsep}{0.15em} 
\centering
  \scalebox{0.95}{
\begin{tabular}{ccccccc}
\addpic{figures/images_st_cow_full/mb_4.png}  & 
\addpic{figures/images_st_cow_full/cow_101.png}  & 
\addpic{figures/images_st_cow_full/cow_102.png}  & 
\addpic{figures/images_st_cow_full/cow_103.png}  & 
\addpic{figures/images_st_cow_full/cow_104.png}  & 
\addpic{figures/images_st_cow_full/cow_105.png}  \\ 
% \addpic{figures/images_st_cow_full/cow_106.png}  & 
% \addpic{figures/images_st_cow_full/cow_107.png}  & 
% \addpic{figures/images_st_cow_full/cow_108.png}  & 
% \addpic{figures/images_st_cow_full/cow_109.png}  & 
% \addpic{figures/images_st_cow_full/cow_110.png}  & 
% \addpic{figures/images_st_cow_full/cow_111.png}  \\ 
\addpic{figures/images_st_cow_full/cow_112.png}  & 
\addpic{figures/images_st_cow_full/cow_113.png}  & 
\addpic{figures/images_st_cow_full/cow_114.png}  & 
\addpic{figures/images_st_cow_full/cow_115.png}  & 
\addpic{figures/images_st_cow_full/cow_116.png}  & 
\addpic{figures/images_st_cow_full/cow_117.png}  \\ 
\addpic{figures/images_st_zebra_full/mb_7.png}  & 
\addpic{figures/images_st_zebra_full/zebra_108.png}  & 
\addpic{figures/images_st_zebra_full/zebra_110.png}  & 
\addpic{figures/images_st_zebra_full/zebra_111.png}  & 
\addpic{figures/images_st_zebra_full/zebra_112.png}  & 
\addpic{figures/images_st_zebra_full/zebra_113.png}  \\ 
\addpic{figures/images_st_zebra_full/zebra_114.png}  & 
\addpic{figures/images_st_zebra_full/zebra_115.png}  & 
\addpic{figures/images_st_zebra_full/zebra_116.png}  & 
\addpic{figures/images_st_zebra_full/zebra_117.png}  & 
\addpic{figures/images_st_zebra_full/zebra_118.png}  & 
\addpic{figures/images_st_zebra_full/zebra_119.png}  \\ 
\addpic{figures/images_st_zebra_full/zebra_120.png}  & 
\addpic{figures/images_st_zebra_full/zebra_121.png}  & 
\addpic{figures/images_st_zebra_full/zebra_122.png}  & 
\addpic{figures/images_st_zebra_full/zebra_123.png}  & 
\addpic{figures/images_st_zebra_full/zebra_124.png}  & 
\addpic{figures/images_st_zebra_full/zebra_106.png} \\
\addpic{figures/images_st_sheep_full/mb_5.png} & 
% \addpic{figures/images_st_sheep_full/sheep_101.png}  & 
% \addpic{figures/images_st_sheep_full/sheep_102.png}  & 
% \addpic{figures/images_st_sheep_full/sheep_100.png}   & 
% \addpic{figures/images_st_sheep_full/sheep_104.png}  & 
% \addpic{figures/images_st_sheep_full/sheep_105.png}  \\ 
% \addpic{figures/images_st_sheep_full/sheep_106.png}  & 
% \addpic{figures/images_st_sheep_full/sheep_118.png}  & 
% \addpic{figures/images_st_sheep_full/sheep_122.png}  & 
% \addpic{figures/images_st_sheep_full/sheep_109.png}  & 
% \addpic{figures/images_st_sheep_full/sheep_110.png}  & 
% \addpic{figures/images_st_sheep_full/sheep_111.png}  \\ 
% \addpic{figures/images_st_sheep_full/sheep_112.png}  & 
\addpic{figures/images_st_sheep_full/sheep_113.png}  & 
\addpic{figures/images_st_sheep_full/sheep_114.png}  & 
\addpic{figures/images_st_sheep_full/sheep_121.png}  & 
\addpic{figures/images_st_sheep_full/sheep_116.png}  & 
\addpic{figures/images_st_sheep_full/sheep_117.png}  \\ 
% \addpic{figures/images_st_sheep_full/sheep_118.png}  & 
% \addpic{figures/images_st_sheep_full/sheep_119.png}  & 
% \addpic{figures/images_st_sheep_full/sheep_120.png}  & 
% \addpic{figures/images_st_sheep_full/sheep_121.png}  & 
% \addpic{figures/images_st_sheep_full/sheep_122.png}  & 
% \addpic{figures/images_st_sheep_full/sheep_123.png}  \\ 
\addpic{figures/images_st_sheep_full/sheep_124.png}  & 
\addpic{figures/images_st_sheep_full/sheep_125.png}  & 
\addpic{figures/images_st_sheep_full/sheep_126.png}  & 
\addpic{figures/images_st_sheep_full/sheep_127.png}  & 
\addpic{figures/images_st_sheep_full/sheep_128.png}  & 
\addpic{figures/images_st_sheep_full/sheep_129.png}  \\ 
\end{tabular}
}
\vspace{-0.1in}
\captionof{figure}{} 
\label{fig:contours2}
\end{table*} 

==> visuals/birds2_c.tex <==
\begin{table*}[!h]
\setlength{\tabcolsep}{0.15em} 
\centering
  \scalebox{0.95}{
\begin{tabular}{ccccccc}
\addpic{figures/images_st_cow_full/mb_contour_4.png}  & 
\addpic{figures/images_st_cow_full/cow_101_contour.png}  & 
\addpic{figures/images_st_cow_full/cow_102_contour.png}  & 
\addpic{figures/images_st_cow_full/cow_103_contour.png}  & 
\addpic{figures/images_st_cow_full/cow_104_contour.png}  & 
\addpic{figures/images_st_cow_full/cow_105_contour.png}  \\ 
% \addpic{figures/images_st_cow_full/cow_106_contour.png}  & 
% \addpic{figures/images_st_cow_full/cow_107_contour.png}  & 
% \addpic{figures/images_st_cow_full/cow_108_contour.png}  & 
% \addpic{figures/images_st_cow_full/cow_109_contour.png}  & 
% \addpic{figures/images_st_cow_full/cow_110_contour.png}  & 
% \addpic{figures/images_st_cow_full/cow_111_contour.png}  \\ 
\addpic{figures/images_st_cow_full/cow_112_contour.png}  & 
\addpic{figures/images_st_cow_full/cow_113_contour.png}  & 
\addpic{figures/images_st_cow_full/cow_114_contour.png}  & 
\addpic{figures/images_st_cow_full/cow_115_contour.png}  & 
\addpic{figures/images_st_cow_full/cow_116_contour.png}  & 
\addpic{figures/images_st_cow_full/cow_117_contour.png}  \\ 
\addpic{figures/images_st_zebra_full/mb_contour_7.png}  & 
\addpic{figures/images_st_zebra_full/zebra_108_contour.png}  & 
\addpic{figures/images_st_zebra_full/zebra_110_contour.png}  & 
\addpic{figures/images_st_zebra_full/zebra_111_contour.png}  & 
\addpic{figures/images_st_zebra_full/zebra_112_contour.png}  & 
\addpic{figures/images_st_zebra_full/zebra_113_contour.png}  \\ 
\addpic{figures/images_st_zebra_full/zebra_114_contour.png}  & 
\addpic{figures/images_st_zebra_full/zebra_115_contour.png}  & 
\addpic{figures/images_st_zebra_full/zebra_116_contour.png}  & 
\addpic{figures/images_st_zebra_full/zebra_117_contour.png}  & 
\addpic{figures/images_st_zebra_full/zebra_118_contour.png}  & 
\addpic{figures/images_st_zebra_full/zebra_119_contour.png}  \\ 
\addpic{figures/images_st_zebra_full/zebra_120_contour.png}  & 
\addpic{figures/images_st_zebra_full/zebra_121_contour.png}  & 
\addpic{figures/images_st_zebra_full/zebra_122_contour.png}  & 
\addpic{figures/images_st_zebra_full/zebra_123_contour.png}  & 
\addpic{figures/images_st_zebra_full/zebra_124_contour.png}  & 
\addpic{figures/images_st_zebra_full/zebra_106_contour.png} \\
\addpic{figures/images_st_sheep_full/mb_contour_5.png} & 
% \addpic{figures/images_st_sheep_full/sheep_101_contour.png}  & 
% \addpic{figures/images_st_sheep_full/sheep_102_contour.png}  & 
% \addpic{figures/images_st_sheep_full/sheep_100_contour.png}   & 
% \addpic{figures/images_st_sheep_full/sheep_104_contour.png}  & 
% \addpic{figures/images_st_sheep_full/sheep_105_contour.png}  \\ 
% \addpic{figures/images_st_sheep_full/sheep_106_contour.png}  & 
% \addpic{figures/images_st_sheep_full/sheep_118_contour.png}  & 
% \addpic{figures/images_st_sheep_full/sheep_122_contour.png}  & 
% \addpic{figures/images_st_sheep_full/sheep_109_contour.png}  & 
% \addpic{figures/images_st_sheep_full/sheep_110_contour.png}  & 
% \addpic{figures/images_st_sheep_full/sheep_111_contour.png}  \\ 
% \addpic{figures/images_st_sheep_full/sheep_112_contour.png}  & 
\addpic{figures/images_st_sheep_full/sheep_113_contour.png}  & 
\addpic{figures/images_st_sheep_full/sheep_114_contour.png}  & 
\addpic{figures/images_st_sheep_full/sheep_121_contour.png}  & 
\addpic{figures/images_st_sheep_full/sheep_116_contour.png}  & 
\addpic{figures/images_st_sheep_full/sheep_117_contour.png}  \\ 
% \addpic{figures/images_st_sheep_full/sheep_118_contour.png}  & 
% \addpic{figures/images_st_sheep_full/sheep_119_contour.png}  & 
% \addpic{figures/images_st_sheep_full/sheep_120_contour.png}  & 
% \addpic{figures/images_st_sheep_full/sheep_121_contour.png}  & 
% \addpic{figures/images_st_sheep_full/sheep_122_contour.png}  & 
% \addpic{figures/images_st_sheep_full/sheep_123_contour.png}  \\ 
\addpic{figures/images_st_sheep_full/sheep_124_contour.png}  & 
\addpic{figures/images_st_sheep_full/sheep_125_contour.png}  & 
\addpic{figures/images_st_sheep_full/sheep_126_contour.png}  & 
\addpic{figures/images_st_sheep_full/sheep_127_contour.png}  & 
\addpic{figures/images_st_sheep_full/sheep_128_contour.png}  & 
\addpic{figures/images_st_sheep_full/sheep_129_contour.png}  \\ 
\end{tabular}
}
\vspace{-0.1in}
\captionof{figure}{} 
\label{fig:contours2}
\end{table*} 

==> visuals/birds_c.tex <==
\begin{table*}[!h]
\setlength{\tabcolsep}{0.15em} 
\centering
  \scalebox{0.95}{
\begin{tabular}{cccccc}
\addpic{figures/images_st_bird_full/mb_contour_2.png}  & 
\addpic{figures/images_st_bird_full/bird_101_contour.png}  & 
\addpic{figures/images_st_bird_full/bird_102_contour.png}  & 
\addpic{figures/images_st_bird_full/bird_103_contour.png}  & 
\addpic{figures/images_st_bird_full/bird_104_contour.png}  & 
\addpic{figures/images_st_bird_full/bird_105_contour.png}  \\ 
\addpic{figures/images_st_bird_full/bird_127_contour.png}  &
\addpic{figures/images_st_bird_full/bird_107_contour.png}  & 
\addpic{figures/images_st_bird_full/bird_108_contour.png}  & 
\addpic{figures/images_st_bird_full/bird_106_contour.png}  & 
\addpic{figures/images_st_bird_full/bird_110_contour.png}  & 
\addpic{figures/images_st_bird_full/bird_111_contour.png}  \\ 
\addpic{figures/images_st_bird_full/bird_112_contour.png}  & 
\addpic{figures/images_st_bird_full/bird_100_contour.png}  & 
\addpic{figures/images_st_bird_full/bird_114_contour.png}  & 
\addpic{figures/images_st_bird_full/bird_115_contour.png}  & 
\addpic{figures/images_st_bird_full/bird_116_contour.png}  & 
\addpic{figures/images_st_bird_full/bird_117_contour.png}  \\ 
% \midrule\\
\addpic{figures/images_st_car_full/mb_contour_9.png}  & 
\addpic{figures/images_st_car_full/car_101_contour.png}  & 
\addpic{figures/images_st_car_full/car_102_contour.png}  & 
\addpic{figures/images_st_car_full/car_103_contour.png}  & 
\addpic{figures/images_st_car_full/car_100_contour.png}   & 
\addpic{figures/images_st_car_full/car_105_contour.png}  \\ 
\addpic{figures/images_st_car_full/car_120_contour.png}  & 
\addpic{figures/images_st_car_full/car_123_contour.png}  & 
\addpic{figures/images_st_car_full/car_108_contour.png}  & 
\addpic{figures/images_st_car_full/car_109_contour.png}  & 
\addpic{figures/images_st_car_full/car_110_contour.png}  & 
\addpic{figures/images_st_car_full/car_111_contour.png}  \\ 
\addpic{figures/images_st_car_full/car_112_contour.png}  & 
\addpic{figures/images_st_car_full/car_113_contour.png}  & 
\addpic{figures/images_st_car_full/car_114_contour.png}  & 
\addpic{figures/images_st_car_full/car_115_contour.png}  & 
\addpic{figures/images_st_car_full/car_116_contour.png}  & 
\addpic{figures/images_st_car_full/car_117_contour.png}  \\ 
% \addpic{figures/images_st_car_full/car_118_contour.png}  & 
% \addpic{figures/images_st_car_full/car_119_contour.png}  & 
% \addpic{figures/images_st_car_full/car_120_contour.png}  & 
% \addpic{figures/images_st_car_full/car_121_contour.png}  & 
% \addpic{figures/images_st_car_full/car_122_contour.png}  & 
% \addpic{figures/images_st_car_full/car_123_contour.png}  \\ 
% \addpic{figures/images_st_car_full/car_124_contour.png}  & 
% \addpic{figures/images_st_car_full/car_125_contour.png}  & 
% \addpic{figures/images_st_car_full/car_126_contour.png}  & 
% \addpic{figures/images_st_car_full/car_127_contour.png}  & 
% \addpic{figures/images_st_car_full/car_128_contour.png}  & 
% \addpic{figures/images_st_car_full/car_129_contour.png}  \\
\addpic{figures/images_st_horse_full/mb_contour_7.png}  & 
\addpic{figures/images_st_horse_full/horse_101_contour.png}  & 
\addpic{figures/images_st_horse_full/horse_102_contour.png}  & 
\addpic{figures/images_st_horse_full/horse_103_contour.png}  & 
\addpic{figures/images_st_horse_full/horse_104_contour.png}  & 
\addpic{figures/images_st_horse_full/horse_105_contour.png}  \\ 
\addpic{figures/images_st_horse_full/horse_100_contour.png} & 
\addpic{figures/images_st_horse_full/horse_107_contour.png}  & 
\addpic{figures/images_st_horse_full/horse_108_contour.png}  & 
\addpic{figures/images_st_horse_full/horse_109_contour.png}  & 
\addpic{figures/images_st_horse_full/horse_110_contour.png}  & 
\addpic{figures/images_st_horse_full/horse_111_contour.png}  \\ 
\end{tabular}
}
\vspace{-0.1in}
\captionof{figure}{} 
\label{fig:qual-results-detection}
\end{table*} 

==> visuals/cartfs.tex <==
\begin{table}[!h]
\setlength{\tabcolsep}{0.15em} 
\centering
  \scalebox{0.95}{
\begin{tabular}{cc}
\addpic{figures/car_tfs/112_img1_kp.png}  & 
\addpic{figures/car_tfs/112_img12.png}\\
\addpic{figures/car_tfs/143_img1_kp.png}  & 
\addpic{figures/car_tfs/143_img12.png}\\
% \addpic{figures/car_tfs/167_img1_kp.png}  & 
% \addpic{figures/car_tfs/167_img12.png}\\
\addpic{figures/car_tfs/180_img1_kp.png}  & 
\addpic{figures/car_tfs/180_img12.png}\\
\end{tabular}
}
\vspace{-0.1in}
\captionof{figure}{} 
\label{fig:kp_transfer_car}
\end{table} 
